DAMe: Personalized Federated Social Event Detection with Dual Aggregation Mechanism

Training social event detection models through federated learning (FedSED) aims to improve participants' performance on the task. However, existing federated learning paradigms are inadequate for achieving FedSED's objective and exhibit limitations in handling the inherent heterogeneity in social data. This paper proposes a personalized federated learning framework with a dual aggregation mechanism for social event detection, namely DAMe. We present a novel local aggregation strategy utilizing Bayesian optimization to incorporate global knowledge while retaining local characteristics. Moreover, we introduce a global aggregation strategy to provide clients with maximum external knowledge of their preferences. In addition, we incorporate a global-local event-centric constraint to prevent local overfitting and ``client-drift''. Experiments within a realistic simulation of a natural federated setting, utilizing six social event datasets spanning six languages and two social media platforms, along with an ablation study, have demonstrated the effectiveness of the proposed framework. Further robustness analyses have shown that DAMe is resistant to injection attacks.

==> backup.tex <==
% 消融实验全部的表
    % \begin{figure}[]
        %     \centering
        %     \includegraphics[width=1.0\linewidth]{Img/abaltion.pdf}
        %     \caption{The illustration of ablation study.}
        %     \label{fig:ablation}
        % \end{figure}

        % \begin{table*}[]
        % \aboverulesep=0ex
        % \belowrulesep=0ex
        % \caption{Results for RQ3.} 
        % \centering
        % \resizebox{1.0\linewidth}{!}{
        % \begin{tabular}{c|ccc|ccc|ccc|ccc}
        % \toprule
        %   & \multirow{2}{*}{BOLA} & \multirow{2}{*}{SEGA} & \multirow{2}{*}{GLECC} & \multicolumn{3}{c|}{English Twitter}          & \multicolumn{3}{c|}{French Twitter}           & \multicolumn{3}{c}{Arabic Twitter}            \\ 
        %   \cline{5-13} 
        %   &                       &                       &                        & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           \\ 
        %   \hline
        % 1 & \ding{51}             & \ding{51}             & \ding{51}              & .76 $\pm$ .00 & .62 $\pm$ .00 & .22 $\pm$ .01 & .77 $\pm$ .00 & .72 $\pm$ .00 & .26 $\pm$ .00 & .87 $\pm$ .00 & .87 $\pm$ .00 & .90 $\pm$ .00 \\
        % 2 & \ding{51}             & \ding{51}             & \ding{55}              & .76 $\pm$ .00 & .62 $\pm$ .00 & .22 $\pm$ .01 & .76 $\pm$ .00 & .71 $\pm$ .00 & .24 $\pm$ .01 & .86 $\pm$ .00 & .86 $\pm$ .00 & .89 $\pm$ .00 \\
        % 3 & \ding{51}             & \ding{55}             & \ding{51}              & .76 $\pm$ .00 & .62 $\pm$ .00 & .22 $\pm$ .01 & .76 $\pm$ .00 & .71 $\pm$ .00 & .26 $\pm$ .01 & .87 $\pm$ .00 & .87 $\pm$ .00 & .90 $\pm$ .00 \\
        % 4 & \ding{55}             & \ding{51}             & \ding{51}              & .73 $\pm$ .00 & .59 $\pm$ .00 & .21 $\pm$ .00 & .73 $\pm$ .00 & .67 $\pm$ .00 & .20 $\pm$ .01 & .84 $\pm$ .00 & .84 $\pm$ .00 & .87 $\pm$ .00 \\
        % % 5 & \ding{51}             & \ding{55}             & \ding{55}              & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 \\
        % % 6 & \ding{55}             & \ding{51}             & \ding{55}              & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 \\
        % % 7 & \ding{55}             & \ding{55}             & \ding{51}              & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 \\
        % 5 & \ding{55}             & \ding{55}             & \ding{55}              & .73 $\pm$ .00 & .58 $\pm$ .00 & .20 $\pm$ .01 & .74 $\pm$ .00 & .68 $\pm$ .00 & .21 $\pm$ .01 & .64 $\pm$ .00 & .64 $\pm$ .00 & .58 $\pm$ .00 \\
        % \hline\hline
        %   & \multicolumn{3}{c|}{Japanese Twitter}                                  & \multicolumn{3}{c|}{German Twitter}           & \multicolumn{3}{c|}{Chinese Weibo}            & \multicolumn{3}{c}{Average}                   \\ 
        %   \cline{2-13} 
        %   & NMI                   & AMI                   & ARI                    & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           \\ 
        %   \hline
        % 1 & .69 $\pm$ .00         & .62 $\pm$ .00         & .35 $\pm$ .02          & .46 $\pm$ .00 & .38 $\pm$ .00 & .08 $\pm$ .00 & .56 $\pm$ .00 & .47 $\pm$ .00 & .19 $\pm$ .02 & .69           & .61           & .33           \\
        % 2 & .68 $\pm$ .00         & .61 $\pm$ .00         & .34 $\pm$ .00          & .45 $\pm$ .00 & .37 $\pm$ .00 & .07 $\pm$ .00 & .56 $\pm$ .00 & .47 $\pm$ .00 & .17 $\pm$ .01 & .68           & .61           & .32           \\
        % 3 & .69 $\pm$ .00         & .62 $\pm$ .00         & .35 $\pm$ .02          & .45 $\pm$ .00 & .37 $\pm$ .01 & .06 $\pm$ .00 & .56 $\pm$ .00 & .47 $\pm$ .00 & .18 $\pm$ .01 & .68           & .61           & .33           \\
        % 4 & .67 $\pm$ .00         & .59 $\pm$ .00         & .31 $\pm$ .02          & .45 $\pm$ .00 & .37 $\pm$ .00 & .07 $\pm$ .01 & .53 $\pm$ .00 & .43 $\pm$ .00 & .12 $\pm$ .00 & .66           & .58           & .30           \\
        % % 5 & .00 $\pm$ .00         & .00 $\pm$ .00         & .00 $\pm$ .00          & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 \\
        % % 6 & .00 $\pm$ .00         & .00 $\pm$ .00         & .00 $\pm$ .00          & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 \\
        % % 7 & .00 $\pm$ .00         & .00 $\pm$ .00         & .00 $\pm$ .00          & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 & .00 $\pm$ .00 \\
        % 5 & .64 $\pm$ .00         & .56 $\pm$ .00         & .18 $\pm$ .01          & .46 $\pm$ .00 & .39 $\pm$ .01 & .08 $\pm$ .01 & .53 $\pm$ .00 & .43 $\pm$ .00 & .11 $\pm$ .00 & .62           & .55           & .23           \\
        % \bottomrule
        % \end{tabular}
        % }
        % \end{table*}


% 消融实验小表
        % \begin{table}[]
        % \aboverulesep=0ex
        % \belowrulesep=0ex
        % \caption{Results for RQ3.} 
        % \centering
        % \setlength{\tabcolsep}{2mm}{
        % % \resizebox{1.0\linewidth}{!}{
        % \begin{tabular}{c|ccc|ccc}
        % \toprule
        %   & \multirow{2}{*}{BOLA} & \multirow{2}{*}{SEGA} & \multirow{2}{*}{GLECC} & \multicolumn{3}{c}{Average}                  \\ 
        %   \cline{5-7} 
        %   &                       &                       &                        & NMI           & AMI           & ARI           \\ 
        %   \hline
        % 1 & \ding{51}             & \ding{51}             & \ding{51}              & .69           & .61           & .33           \\
        % 2 & \ding{51}             & \ding{51}             & \ding{55}              & .68           & .61           & .32           \\
        % 3 & \ding{51}             & \ding{55}             & \ding{51}              & .68           & .61           & .33           \\
        % 4 & \ding{55}             & \ding{51}             & \ding{51}              & .66           & .58           & .30           \\
        % 5 & \ding{55}             & \ding{55}             & \ding{55}              & .62           & .55           & .23           \\
        % \bottomrule
        % \end{tabular}
        % }
        % \label{tab:rq3}
        % \end{table}





        
         % 在服务器端，我们基于二维结构熵提出了一个新的个性化联邦融合算法，目的是为每个client分配个性化的全局模型。其中，我们通过最小化二维结构熵进一步将用户节点进行分组，缓解不同客户端数据间非独立同分布的问题。我们的结构熵个性化融合策略步骤如下：
        % We can formulate the problem of aggregating the weights of the global model $\Theta_g^r$
        
        % \paragraph{\textbf{Graph Pooling}}
        % % 在使用结构熵进行个性化联邦学习之前，我们需要构建client之间的相似度，在本文中，我们设定了一个public data用于服务器端获取客户端之间的分布相似度。为了获取客户端间的相似度，我们随机从public data中采样messages，并构建成相应的图。通过graph pooling操作，我们得到不同客户端在当前graph的表示，用于计算client相似度。
        % Before applying structural entropy for personalized federated learning, we need to establish the similarity between clients. In this paper, we define a public dataset for the server to acquire the distribution similarity between clients. To obtain the similarity between clients, we randomly sample messages from the public dataset and construct corresponding graphs. Through graph pooling operations, we obtain representations of different clients in the current graph, which are used to calculate client similarity.
        % \begin{equation}
        %     P(G) = \frac{1}{N} \sum_{i=1}^N h_i,
        % \end{equation}
        % Here, $h_u$  represents the embedding vector of node $u$ .
        % The similarity between two functions defined by GNNs at clients \( i \) and \( j \) is then defined as follows:
        % \begin{equation}
        %     S(i, j) = \frac{\tilde{h}_i \cdot \tilde{h}_j}{\|\tilde{h}_i\| \|\tilde{h}_j\|},
        % \end{equation}
        % where \( \tilde{h} \) is the averaged output of all node embeddings for input \( \tilde{G} \) with an average operation.



        % Given a directed graph $G_{client} = (V, E)$ with $K$ clients, suppose that a weight function defines the weights assigned to edges $ \omega: E \to \mathbb{R}^{+}$. 
        % Define the weighted degree of node $u$ to be $d_u = \sum_{v \in N(u)} \omega((u,v))$, where $N(u)$ is the set of neighbors of $u$.
        % The local model parameter is represented as  $\Theta_u$, and the personalized global model for client $u$ is denoted as $\hat{\Theta}_u$.
        % We can formulate the problem of personalized federated learning through the following optimization problem,
        % \begin{equation}
        %     \hat{\Theta}_u = \sum_{v=1}^{N(u)} \alpha_{uv} \cdot \Theta_{v}, \quad
        %     \alpha_{uv} = \frac{\exp(\tau \cdot S(u,v))}{\sum_{k} \exp(\tau \cdot S(u,k))},
        % \end{equation}
        % where $\alpha_{uv}$ is a normalized similarity between clients $u$ and $v$, and $\tau$ is a hyperparameter for scaling the unnormalized similarity score.



        
        
        % % wyf
        % Let $G_{client} = (V, E)$ represent a client graph constructed from the distribution correlation of data across various platforms. Suppose $\mathcal{P} = \{X_1, X_2, \dots, X_L\}$ forms a partition of $V$, where each $X_i$ constitutes a message cluster containing detected events. A faithful decoding of message correlations in $G$ assigns related messages to the same cluster and unrelated ones to different clusters. To achieve this goal, we employ 2D structural entropy minimization \cite{}, which mitigates noise stemming from non-independent identically distributed (non-IID) data across different platforms. Additionally, it dynamically facilitates personalized federated fusion without prior knowledge of client data distribution correlations. 


        % 在这里，我们先给出图G的二维结构熵计算公式【cite】：
        % \begin{equation}
        %     \begin{aligned} 
        %     \mathcal{H}^2(G)= & \sum_{j=1}^L \frac{v_j}{\operatorname{vol}(G)} \cdot H\left(\frac{d_1^{(j)}}{v_j}, \ldots, \frac{d_{n_j}^{(j)}}{v_j}\right) -\frac{g_j}{\operatorname{vol}(G)} \log _2 \frac{v_j}{\operatorname{vol}(G)} \\ = & -\sum_{j=1}^L \frac{v_j}{\operatorname{vol}(G)} \sum_{i=1}^{n_j} \frac{d_i^{(j)}}{v_j} \log _2 \frac{d_i^{(j)}}{v_j} + \frac{g_j}{\operatorname{vol}(G)} \log _2 \frac{v_j}{\operatorname{vol}(G)},
        %     \end{aligned}
        % \end{equation}
        % 其中L是G中的簇数量，$d_i$是节点i的所有边权重之和，。。。（一样的解释）。
        % 具体来说，在我们所构建的客户端图中，每个节点最开始便是一个簇。我们通过贪婪的最小化二维结构熵策略【cite Angsheng Li 2016（应该是）】来分区。
        % 对于给定的任意两个簇$c_i$ 和 $c_j$，它们合并为一个簇($c_k$)前后的2D SE 的差值为：
        % \begin{equation}
        %     \begin{aligned} 
        %            \Delta SE= & SE_{new}-SE_{old} 
        %                     =  H^P_{c_k} - H^2_{c_i} - H^2_{c_j}\\
        %                     = & - \frac{g_k}{\operatorname{vol}(G)}\log _2 \frac{v_k}{\operatorname{vol}(G)} - \sum_{x=1}^{n_k} \frac{d_x}{\operatorname{vol}(G)}\log _2 \frac{d_x}{v_k}\\
        %                     & + \frac{g_i}{\operatorname{vol}(G)}\log _2 \frac{v_i}{\operatorname{vol}(G)} + \sum_{x=1}^{n_i} \frac{d_x}{\operatorname{vol}(G)}\log _2 \frac{d_x}{v_i}\\
        %                     & + \frac{g_j}{\operatorname{vol}(G)}\log _2 \frac{v_j}{\operatorname{vol}(G)} + \sum_{x=1}^{n_j} \frac{d_x}{\operatorname{vol}(G)}\log _2 \frac{d_x}{v_j}\\
        %                     = & - \frac{g_k}{\operatorname{vol}(G)}\log _2 \frac{v_k}{\operatorname{vol}(G)}
        %                      + \frac{g_i}{\operatorname{vol}(G)}\log _2 \frac{v_i}{\operatorname{vol}(G)}\\
        %                      & + \frac{g_j}{\operatorname{vol}(G)}\log _2 \frac{v_j}{\operatorname{vol}(G)}
        %                      + \frac{v_i}{\operatorname{vol}(G)}\log _2 \frac{v_k}{v_i}\\
        %                      & + \frac{v_j}{\operatorname{vol}(G)}\log _2 \frac{v_k}{v_j},
        %     \end{aligned}
        % \end{equation}
        % 需要注意的是，我们始终合并 ΔSE最小的两个簇，直到没有ΔSE<0时，代表2D SE已经无法减小了，此时我们也获得了最终的分区结果。
        % 接下来，我们根据分区结果针对每个客户端融合它个性化的全局模型。
        % 在这里，我们认为某个簇中的客户端是具有关联的，给定一个客户端$C_i$,它与自己的相似度为1，而与簇内的其他客户端的相似度依旧由两者间边的权重决定。
        % 将这些权重进行softmax操作后，就得到了针对$C_i$的每个相关联客户端的参数权重，我们按照该权重便融合得到了全局模型：
        % 
        % $d_i^{(j)}$ stands for the degree of the $i$-th node of $X_j$,



        
        % We define the weighted degree of node $u$ in cluster $X_j$ as follows:
        % \begin{equation}
        %     d_u^{(j)} = \sum_{v \in N(u)} \omega((u,v)), 
        % \end{equation}
        % where $N(u)$ denotes the set of neighbors of $u$ in $X_j$.
        % And the structural information of $G_{\text{client}}$ by $\mathcal{P} $ is defined as:
        % \begin{equation}
        % \begin{aligned} 
        % % 这里{\text{client}} 回头准备换一个符合，公式里太罗嗦了
        % \mathcal{H}^{\mathcal{P}}(G)= & \sum_{j=1}^L \frac{V_j}{\operatorname{vol}(G)} \cdot H\left(\frac{d_1^{(j)}}{V_j}, \ldots, \frac{d_{n_j}^{(j)}}{V_j}\right) \\ & -\sum_{j=1}^L \frac{g_j}{\operatorname{vol}(G)} \log _2 \frac{V_j}{\operatorname{vol}(G)} \\ = & -\sum_{j=1}^L \frac{V_j}{\operatorname{vol}(G)} \sum_{i=1}^{n_j} \frac{d_i^{(j)}}{V_j} \log _2 \frac{d_i^{(j)}}{V_j} \\ & -\sum_{j=1}^L \frac{g_j}{\operatorname{vol}(G)} \log _2 \frac{V_j}{\operatorname{vol}(G)},
        % \end{aligned}
        % \end{equation}
        % where $L$ denotes the number of clusters in partition $\mathcal{P}$, $n_j$ represents the number of nodes in cluster $X_j$,  $V_j$ computed by the function $vol(\cdot)$ indicates the volume of cluster $X_j$, and $g_j$ signifies the sum of weights of edges with exactly one endpoint in cluster $X_j$.


        % For each client $u \in V$, the personalized model $\hat{\Theta}_u$ can be denoted through the following formula:
        % \begin{equation}
        % \hat{\Theta}_u = \sum_{v \in N(u)} \alpha_{uv} \cdot \Theta_{v}, \quad
        % \alpha_{uv} = \frac{\exp(\tau \cdot S(u,v))}{\sum_{k} \exp(\tau \cdot S(u,k))},
        % \end{equation}
        % where $\alpha_{uv}$ is a normalized similarity between clients $u$ and $v$, and $\tau$ is a hyperparameter for scaling the unnormalized similarity score.  




         % \textbf{Model Poisoning Attack.}
        % % We measure the performance drop $\boldsymbol{\Delta}$NMI on the task SED. 
        % % This drop serves as an indication of the impact of the poisoned model on the performance of the clean participants.
        % We assess the impact of the model poisoning attack by measuring the performance disparity $\boldsymbol{\Delta}\text{\textbf{NMI}}$ between the clean scenario and the poisoned scenario:
        % \begin{equation}
        %     \boldsymbol{\Delta}\text{NMI}= \text{NMI}_{clean} - \text{NMI}_{poisoned}.
        % \end{equation}

        % \textbf{Data Poisoning Attack.}
        % In addition to $\boldsymbol{\Delta}\text{\textbf{NMI}}$, we also calculate the Attack Success Rate (\textbf{ASR}) on poisoned samples in the testing set.
        % Firstly, assuming the backdoor was successfully implanted, the poisoned samples are expected to belong to the same cluster. 
        % Based on this assumption, we assess the NMI between the clustering results of the poisoned samples and their true labels.
        % If the poisoning attack is successful, the NMI value should be low (indicating that the clustering results show them belonging to the same cluster while their true labels are inconsistent). 
        % Otherwise, the NMI value would be higher.
        % Therefore, the ASR is calculated as:
        % \begin{equation}
        %     \text{ASR} = 1 - \text{NMI}_{poisoned\_samples}.
        % \end{equation}



        
    % \subsection{Graph Neural Networks}\label{sec:gnn}
    %     Given a graph $G=(V, E)$, consisting of a set of nodes $V$ and edges $E$.
    %     GNNs \cite{wu2020comprehensive} represent nodes based on themselves and their neighbors at the $l$-th layer by:      
    %     \begin{equation}
    %         \begin{split}
    %             \boldsymbol{H}^{(l)}_v &= \text{UPD}^{(l-1)}\left(\boldsymbol{H}_v^{(l-1)}, \boldsymbol{a}_v^{(l-1)}\right), \\
    %             \boldsymbol{a}_v^{(l-1)} =& \text{AGG}^{(l-1)}\left(\{\boldsymbol{H}_u^{(l-1)}:\forall u \in \mathcal{N}\left(v\right)\}\right),
    %         \end{split}
    %     \end{equation}
    %     where $\boldsymbol{H}^{(l)}_v$ denotes the representation of node $v$ at the $l$-th layer, $\mathcal{N}(v)$ denotes the set of neighbors of node $v$.
    %     AGG and UDP refer to the aggregate and update strategies for neighbor aggregation and node update, respectively.  



    % In FedSED, the objective is for the local model to achieve better performance on private data by integrating knowledge from the global.
        % Therefore, the objective of client $k$ is as follows:
        % \begin{equation}
        %     \underset{\theta_{l_k}, \theta_g}{\arg \min} \mathcal{L}(\theta_{l_k}) = \frac{1}{N_k} \sum_{i=1}^{N_k} \mathcal{L}(\mathcal{D}_k; [\lambda \cdot\theta_{l_k} + (1-\lambda) \cdot\theta_g]),
        % \end{equation}
        % where $\lambda$ is the local aggregation weight.



        % \paragraph{\textbf{Federated Social Event Detection}}
        % Given a network of decentralized social platforms, each holding a collection of social messages $M^{k}$ where $k$ denotes platform $k$, and the $i$-th message is represented as $m_i^{k} = \{d_i^{k}, t_i^{k}, a_i^{k}\}$, where $d_i^{k}$, $t_i^{k}$, and $a_i^{k}$ denote the text document, timestamp, and attributes (such as hashtags, users, entities) of $m_i^{k}$.
        % A federated social event detection algorithm aims to collaboratively learn a global model $f(M^{1}, M^{2}, ..., M^{K}; \theta^g) = E$, where $\theta^g$ represents the global model parameters, and $E = \{e_j \mid 1 \leq j \leq |E|\}$ is the set of detected events across all sources. This algorithm respects the data privacy and security constraints of individual sources by training the global model using decentralized computation on local data while preserving data confidentiality.



        % PP-GCN \cite{peng2019fine} leverages multiple attributes through carefully designed meta-paths and designs a pairwise loss to learn representation yield from Graph Convolutional Networks (GCN).
        % QSGNN \cite{ren2022known} designs a contrastive learning-based pairwise loss to constrain intra- and inter-event message representations learned from GNNs.
        % In Ditto \cite{li2021ditto}, a personalized model is learned on the client side, aided by a proximal term for gathering information from the server.
        % For example, \citet{liu2023communication} proposes using adapters to facilitate client information exchange without needing identical model structures.


        % \begin{table}[htbp]
        % \aboverulesep=0ex
        % \belowrulesep=0ex
        % \caption{Average results of ablation study.} 
        % \centering
        % \setlength{\tabcolsep}{3mm}{
        % % \resizebox{1.0\linewidth}{!}{
        % \begin{tabular}{l|ccc}
        % \toprule
        %                                  & \multicolumn{3}{c}{Average} \\
        % \cline{2-4} 
        %                                  & NMI   & AMI   & ARI         \\ 
        % \hline
        % DAMe                             & .68   & .60   & .30         \\
        % \multicolumn{1}{r|}{w/o GLECC}   & .67   & .60   & .30         \\
        % \multicolumn{1}{r|}{w/o SEGA}    & .67   & .59   & .29         \\
        % \multicolumn{1}{r|}{w/o BOLA}    & .65   & .58   & .28         \\
        % \multicolumn{1}{r|}{w/o all}     & .62   & .55   & .23         \\
        % \bottomrule
        % \end{tabular}
        % }
        % \label{tab:ablation}
        % \end{table}



        % \begin{table*}[htbp]
        % \aboverulesep=0ex
        % \belowrulesep=0ex
        % \caption{Results for RQ1.} 
        % \centering
        % \resizebox{1.0\linewidth}{!}{
        % \begin{tabular}{l|ccc|ccc|ccc|ccc}
        % \toprule
        % Clients    & \multicolumn{3}{|c|}{English Twitter}         & \multicolumn{3}{|c|}{French Twitter}          & \multicolumn{3}{|c|}{Arabic Twitter}          & \multicolumn{3}{|c}{Japanese Twitter}              \\
        % \hline
        % Metrics    & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           & NMI           & AMI           & ARI                \\
        % \hline
        % Local      & .69 $\pm$ .00 & .52 $\pm$ .00 & .13 $\pm$ .00 & .69 $\pm$ .00 & .62 $\pm$ .00 & .15 $\pm$ .00 & .55 $\pm$ .00 & .55 $\pm$ .00 & .50 $\pm$ .00 & .60 $\pm$ .00 & .50 $\pm$ .00 & .11 $\pm$ .01      \\
        % \hline
        % FedAvg     & .73 $\pm$ .00 & .58 $\pm$ .00 & .20 $\pm$ .01 & .74 $\pm$ .00 & .68 $\pm$ .00 & .21 $\pm$ .01 & .64 $\pm$ .00 & .64 $\pm$ .00 & .58 $\pm$ .00 & .64 $\pm$ .00 & .56 $\pm$ .00 & .18 $\pm$ .01      \\
        % FedProx    & .71 $\pm$ .00 & .55 $\pm$ .00 & .16 $\pm$ .00 & .70 $\pm$ .00 & .64 $\pm$ .00 & .17 $\pm$ .00 & .59 $\pm$ .01 & .59 $\pm$ .01 & .54 $\pm$ .02 & .62 $\pm$ .00 & .53 $\pm$ .00 & .14 $\pm$ .01      \\
        % \hline
        % Per-FedAvg & .72 $\pm$ .00 & .56 $\pm$ .00 & .17 $\pm$ .01 & .70 $\pm$ .00 & .64 $\pm$ .00 & .18 $\pm$ .01 & .62 $\pm$ .01 & .62 $\pm$ .00 & .57 $\pm$ .00 & .62 $\pm$ .00 & .53 $\pm$ .00 & .15 $\pm$ .01      \\
        % Ditto      & .73 $\pm$ .00 & .58 $\pm$ .00 & .20 $\pm$ .01 & .73 $\pm$ .00 & .68 $\pm$ .00 & .21 $\pm$ .01 & .63 $\pm$ .02 & .62 $\pm$ .02 & .55 $\pm$ .02 & .64 $\pm$ .00 & .56 $\pm$ .00 & .18 $\pm$ .01      \\
        % SFL        & .69 $\pm$ .00 & .52 $\pm$ .00 & .12 $\pm$ .00 & .69 $\pm$ .00 & .62 $\pm$ .00 & .15 $\pm$ .00 & .56 $\pm$ .00 & .56 $\pm$ .00 & .50 $\pm$ .01 & .60 $\pm$ .00 & .50 $\pm$ .00 & .11 $\pm$ .00      \\
        % APPLE      & .71 $\pm$ .00 & .55 $\pm$ .00 & .16 $\pm$ .01 & .70 $\pm$ .00 & .63 $\pm$ .00 & .16 $\pm$ .00 & .70 $\pm$ .00 & .69 $\pm$ .00 & .73 $\pm$ .00 & .61 $\pm$ .00 & .52 $\pm$ .00 & .12 $\pm$ .00      \\
        % FedALA     & .74 $\pm$ .00 & .59 $\pm$ .00 & .21 $\pm$ .00 & .74 $\pm$ .00 & .69 $\pm$ .00 & .22 $\pm$ .00 & .63 $\pm$ .00 & .63 $\pm$ .00 & .57 $\pm$ .00 & .65 $\pm$ .00 & .56 $\pm$ .00 & .20 $\pm$ .01      \\ 
        % \hline
        % DAMe       & .75 $\pm$ .00 & .61 $\pm$ .00 & .21 $\pm$ .00 & .76 $\pm$ .00 & .70 $\pm$ .00 & .23 $\pm$ .02 & .86 $\pm$ .00 & .86 $\pm$ .00 & .89 $\pm$ .00 & .67 $\pm$ .00 & .59 $\pm$ .00 & .25 $\pm$ .01      \\ 
        % promotion  & $\uparrow$.01 & $\uparrow$.02 & $\uparrow$.01 & $\uparrow$.02 & $\uparrow$.01 & $\uparrow$.01 & $\uparrow$.16 & $\uparrow$.17 & $\uparrow$.16 & $\uparrow$.02 & $\uparrow$.03 & $\uparrow$.05      \\
        % w/o GLECC  & .74 $\pm$ .00 & .60 $\pm$ .00 & .21 $\pm$ .02 & .74 $\pm$ .00 & .69 $\pm$ .00 & .22 $\pm$ .01 & .86 $\pm$ .00 & .86 $\pm$ .00 & .88 $\pm$ .00 & .66 $\pm$ .00 & .59 $\pm$ .00 & .24 $\pm$ .02      \\ 
        % w/o BOLA   & .74 $\pm$ .00 & .60 $\pm$ .00 & .20 $\pm$ .01 & .74 $\pm$ .00 & .69 $\pm$ .00 & .22 $\pm$ .01 & .77 $\pm$ .00 & .77 $\pm$ .00 & .80 $\pm$ .00 & .65 $\pm$ .00 & .57 $\pm$ .00 & .21 $\pm$ .01      \\ 
        % w/o SEGA   & .75 $\pm$ .00 & .61 $\pm$ .00 & .21 $\pm$ .01 & .75 $\pm$ .00 & .70 $\pm$ .00 & .21 $\pm$ .01 & .80 $\pm$ .01 & .80 $\pm$ .01 & .84 $\pm$ .01 & .67 $\pm$ .00 & .59 $\pm$ .00 & .25 $\pm$ .00      \\ 
        % \hline\hline
        % Clients    & \multicolumn{3}{|c|}{German Twitter}          & \multicolumn{3}{|c|}{Chinese Weibo}           & \multicolumn{3}{|c|}{Average}                 & \multicolumn{3}{|c}{Avg. Gain (compare to Local)}  \\
        % \hline
        % Metrics    & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           & NMI           & AMI           & ARI           & NMI           & AMI           & ARI                \\
        % \hline
        % Local      & .41 $\pm$ .00 & .32 $\pm$ .00 & .04 $\pm$ .00 & .47 $\pm$ .00 & .34 $\pm$ .00 & .05 $\pm$ .00 & .57           & .48           & .16           & -             & -             & -                  \\
        % \hline
        % FedAvg     & .46 $\pm$ .00 & .39 $\pm$ .01 & .08 $\pm$ .01 & .53 $\pm$ .00 & .43 $\pm$ .00 & .11 $\pm$ .00 & .62           & .55           & .23           & .04           & .06           & .07                \\
        % FedProx    & .43 $\pm$ .00 & .35 $\pm$ .00 & .06 $\pm$ .00 & .48 $\pm$ .00 & .37 $\pm$ .00 & .07 $\pm$ .00 & .59           & .51           & .19           & .02           & .03           & .03                \\
        % \hline
        % Per-FedAvg & .44 $\pm$ .00 & .36 $\pm$ .00 & .06 $\pm$ .00 & .49 $\pm$ .00 & .38 $\pm$ .00 & .08 $\pm$ .01 & .60           & .51           & .20           & .02           & .03           & .04                \\
        % Ditto      & .46 $\pm$ .00 & .39 $\pm$ .00 & .08 $\pm$ .00 & .53 $\pm$ .00 & .43 $\pm$ .00 & .11 $\pm$ .01 & .62           & .54           & .22           & .04           & .06           & .07                \\
        % SFL        & .41 $\pm$ .00 & .32 $\pm$ .00 & .04 $\pm$ .00 & .47 $\pm$ .00 & .35 $\pm$ .00 & .05 $\pm$ .00 & .57           & .48           & .16           & .00           & .00           & .00                \\
        % APPLE      & .43 $\pm$ .00 & .35 $\pm$ .00 & .06 $\pm$ .00 & .48 $\pm$ .00 & .36 $\pm$ .00 & .06 $\pm$ .00 & .61           & .52           & .22           & .01           & .02           & .01                \\
        % FedALA     & .46 $\pm$ .00 & .39 $\pm$ .00 & .08 $\pm$ .00 & .53 $\pm$ .00 & .43 $\pm$ .00 & .12 $\pm$ .01 & .63           & .55           & .23           & .05           & .06           & .09                \\ 
        % \hline
        % DAMe       & .48 $\pm$ .00 & .40 $\pm$ .00 & .09 $\pm$ .00 & .56 $\pm$ .00 & .46 $\pm$ .00 & .16 $\pm$ .01 & .68           & .60           & .30           & .07           & .09           & .14                \\ 
        % promotion  & $\uparrow$.02 & $\uparrow$.01 & $\uparrow$.01 & $\uparrow$.03 & $\uparrow$.03 & $\uparrow$.04 & $\uparrow$.05 & $\uparrow$.05 & $\uparrow$.07 & $\uparrow$.02 & $\uparrow$.03 & $\uparrow$.05      \\
        % w/o GLECC  & .47 $\pm$ .00 & .40 $\pm$ .00 & .09 $\pm$ .01 & .55 $\pm$ .00 & .46 $\pm$ .00 & .15 $\pm$ .01 & .67           & .60           & .30           & .06           & .09           & .13                \\ 
        % w/o BOLA   & .46 $\pm$ .00 & .39 $\pm$ .00 & .09 $\pm$ .00 & .55 $\pm$ .00 & .45 $\pm$ .00 & .16 $\pm$ .01 & .65           & .58           & .28           & .05           & .07           & .10                \\ 
        % w/o SEGA   & .47 $\pm$ .00 & .40 $\pm$ .00 & .08 $\pm$ .00 & .55 $\pm$ .00 & .45 $\pm$ .00 & .15 $\pm$ .01 & .67           & .59           & .29           & .07           & .09           & .14                \\ 
        % \bottomrule
        % \end{tabular}
        % }
        % \label{tab:rq1}
        % \end{table*}


        % \begin{equation}
        %     \begin{aligned} 
        %        \Delta SE= & SE_{new}-SE_{old} 
        %                 =  H_{X_l}^\mathcal{P} - H_{X_i}^\mathcal{P} - H_{X_j}^\mathcal{P}\\
        %                 = & - \frac{g_l}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(G)} - \sum_{x=1}^{n_l} \frac{d_x}{\operatorname{vol}(G)}\log _2 \frac{d_x}{\operatorname{vol}(X_l)}\\
        %                 & + \frac{g_i}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_i)}{\operatorname{vol}(G)} + \sum_{x=1}^{n_i} \frac{d_x}{\operatorname{vol}(G)}\log _2 \frac{d_x}{\operatorname{vol}(X_i)}\\
        %                 & + \frac{g_j}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_j)}{\operatorname{vol}(G)} + \sum_{x=1}^{n_j} \frac{d_x}{\operatorname{vol}(G)}\log _2 \frac{d_x}{\operatorname{vol}(X_j)}\\
        %                 = & - \frac{g_l}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(G)}
        %                  + \frac{g_i}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_i)}{\operatorname{vol}(G)}\\
        %                  & + \frac{g_j}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_j)}{\operatorname{vol}(G)}
        %                  + \frac{\operatorname{vol}(X_i)}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(X_i)}\\
        %                  & + \frac{\operatorname{vol}(X_j)}{\operatorname{vol}(G)}\log _2 \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(X_j)}.
        %     \end{aligned}
        % \end{equation}




        % the connection for them operation is performed, resulting in the following outcome.
         % 给定一个具体的簇（分区）$X_i$,对于$X_i$中的所有客户端节点，它与自己的相似度为1，而与簇内的其他客户端的相似度为两者间边的权重。
        % 将所有权重进行softmax操作后，就得到了针对$C_j$($C_j \in X_i$)的每个相关联客户端的参数权重，我们按照该权重便融合得到了全局模型：
        % Given a specific partition $X_i$, for all client nodes within $X_i$, the similarity between a client node and itself is 1, while the similarity between a client node and other client nodes within the same cluster is determined by the edge weight between them.
        % By applying the softmax operation to all the weights, we obtain the parameter weights for each associated client node with respect to $C_j$ ($C_j \in X_i$). Using these weights, we fuse the client nodes to obtain the global model:lll
        % For each client $u \in V$, the personalized model $\hat{\Theta}_u$ can be denoted through the following formula:
        % \begin{equation}
        % \hat{\Theta}_u = \sum_{v \in N(u)} \alpha_{uv} \cdot \Theta_{v}, \quad
        % \alpha_{uv} = \frac{\exp(\tau \cdot S(u,v))}{\sum_{k} \exp(\tau \cdot S(u,k))},
        % \end{equation}
        % where $\alpha_{uv}$ is a normalized similarity between clients $u$ and $v$, and $\tau$ is a hyperparameter for scaling the unnormalized similarity score.  
        % $d_i^{(j)}$ stands for the degree of the $i$-th node of $X_j$,



        % \begin{equation}
        %     \alpha_{uv} = \frac{\exp(\tau \cdot S(u,v))}{\sum_{k} \exp(\tau \cdot S(u,k))}.
        % \end{equation}


                % The 2DSE of graph $G$ is calculated as follows \cite{cao2024hierarchical,li2016structural}:
        % \begin{equation}
        %     \begin{aligned} 
        %     \mathcal{H}^\mathcal{P}(G)
        %     = & \sum_{l=1}^L \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(G)} \cdot H\left(\frac{d_1^{(l)}}{\operatorname{vol}(X_l)}, \ldots, \frac{d_{n_l}^{(l)}}{\operatorname{vol}(X_l)}\right)\\ 
        %     & -\sum_{l=1}^L \frac{g_l}{\operatorname{vol}(G)} \log _2 \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(G)} \\ 
        %     = & -\sum_{l=1}^L \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(G)} \sum_{i=1}^{n_l} \frac{d_i^{(l)}}{\operatorname{vol}(X_l)} \log _2 \frac{d_i^{(l)}}{\operatorname{vol}(X_l)} \\
        %     & - \sum_{l=1}^L\frac{g_l}{\operatorname{vol}(G)} \log _2 \frac{\operatorname{vol}(X_l)}{\operatorname{vol}(G)},
        %     \end{aligned}
        % \label{eq:2dse}
        % \end{equation}
